Quantum Advantage from One-Way Functions

We demonstrate quantum advantage with several basic assumptions, specifically based on only the existence of OWFs. We introduce inefficient-verifier proofs of quantumness (IV-PoQ), and construct it from classical bit commitments. IV-PoQ is an interactive protocol between a verifier and a quantum prover consisting of two phases. In the first phase, the verifier is probabilistic polynomial-time, and it interacts with the prover. In the second phase, the verifier becomes inefficient, and makes its decision based on the transcript of the first phase. If the prover is honest, the inefficient verifier accepts with high probability, but any classical malicious prover only has a small probability of being accepted by the inefficient verifier. Our construction demonstrates the following results: (1)If one-way functions exist, then IV-PoQ exist. (2)If distributional collision-resistant hash functions exist (which exist if hard-on-average problems in $\mathbf{SZK}$ exist), then constant-round IV-PoQ exist. We also demonstrate quantum advantage based on worst-case-hard assumptions. We define auxiliary-input IV-PoQ (AI-IV-PoQ) that only require that for any malicious prover, there exist infinitely many auxiliary inputs under which the prover cannot cheat. We construct AI-IV-PoQ from an auxiliary-input version of commitments in a similar way, showing that (1)If auxiliary-input one-way functions exist (which exist if $\mathbf{CZK}\not\subseteq\mathbf{BPP}$), then AI-IV-PoQ exist. (2)If auxiliary-input collision-resistant hash functions exist (which is equivalent to $\mathbf{PWPP}\nsubseteq \mathbf{FBPP}$) or $\mathbf{SZK}\nsubseteq \mathbf{BPP}$, then constant-round AI-IV-PoQ exist.

==> Qextention.tex <==
\section{}
\mor{kakikake}
The following conjecture is exactly the same as \cref{thm:impossible_reduction_formal}
except that $\mathcal{R}$ is not PPT but QPT.
\begin{conjecture}
Let $\Pi$ be a two-round AI-IV-PoQ that satisfies $c$-completeness and $s$-soundness where $c(\secp)-s(\secp)\ge 1/\poly(\secp)$ 
and let $(\mathcal{C},t)$ be a game-based assumption. 
Suppose that there is an oracle-aided $\mathbf{QPT}$ machine $\mathcal{R}$ (the reduction algorithm) such that for any (possibly unbounded-time stateless) randomized classical machine $\cP^*$ that breaks $s$-soundness of $\Pi$, 
$|\Pr[1\gets \langle\mathcal{R}^{\cP^*}(1^\secp),\mathcal{C}(1^\secp) \rangle]-t|$ is non-negligible. 
Then the game-based assumption $(\mathcal{C},t)$ does not hold against quantum adversaries.  
\end{conjecture}

We have the following result.
\begin{theorem}
If quantumly-secure QE-OWFs do not imply quantumly-secure infinitely-often (classical) OWFs, then    
the above conjecture is wrong.
\end{theorem}

\begin{proof}
Assume that the above conjecture is correct.
Then, we show that
quantumly-secure QE-OWFs imply quantumly-secure infinitely-often OWFs. 

If quantumly-secure QE-OWFs exist, then
two-round QV-PoQ exist or quantumly-secure infinitely-often OWFs exist.
Assume that two-round QV-PoQ exist. Then, due to the conjecture,  
the quantumly-secure QE-OWFs are not quantumly-secure, which is the contradiction.
Therefore,
quantumly-secure infinitely-often OWFs exist.
\end{proof}

==> amplification.tex <==
\section{Amplification}
\label{sec:amplification}
\mor{kakikake}

\begin{definition}[Weak OWSGs]
A OWSG is called a weak OWSG if the security definition is replaced with the following one:
There exists a polynomial $p$ such that for any QPT adversary $\cA$ and any polynomial $t$,
\begin{eqnarray*}
\Pr[\top\gets\Ver(k',\phi_k):k\gets\Gen_1(1^\secp),\phi_k\gets\Gen_2(k),k'\gets\cA(\phi_k^{\otimes t})]
\le 1-\frac{1}{p}.
\end{eqnarray*}
\end{definition}

\begin{theorem}
If weak OWSGs exist, then (standard) OWSGs exist.
\end{theorem}

\begin{proof}
Let $(\mathsf{W}.\Gen_1,\mathsf{W}.\Gen_2,\mathsf{W}.\Ver)$ be a weak OWSG.
From it, we construct a (standard) OWSG as follows.
\begin{itemize}
    \item 
    $\Gen_1(1^\secp)\to k:$ Run $k\gets\mathsf{W}.\Gen_1$ $r$ times. Output $k\coloneqq(k_1,k_2,...,k_l)$.
    \item
   $\Gen_2(k)\to\phi_k:$ Parse $k=(k_1,...,k_r)$. Run $\phi_{k_i}\gets\mathsf{W}.\Gen_2(k_i)$ for each $i\in[1,2,...,r]$. 
   Output $\phi_k\coloneqq \phi_{k_1}\otimes...\otimes\phi_{k_r}$.
\item
$\Ver(k',\phi_k)\to\top/\bot:$
Parse $k'=(k'_1,...,k'_r)$. Parse $\phi_k=\phi_{k_1}\otimes...\otimes\phi_{k_r}$.
Run $\mathsf{W}.\Ver(k'_i,\phi_{k'})$ for each $i\in[1,2,...,r]$.
If all results are $\top$, output $\top$.
Otherwise, output $\bot$.
\end{itemize}
The correctness is clear. Assume that it is not secure.
Then, there exists a QPT adversary $\cA$, a polynomial $t$, and a polynomial $p$ such that
\begin{eqnarray*}
\Pr[\top\gets\Ver(k',\phi_k):k\gets\Gen_1(1^\secp),\phi_k\gets\Gen_2(k),k'\gets\cA(\phi_k^{\otimes t})]
\ge \frac{1}{p}.
\end{eqnarray*}




\end{proof}

==> backup1.tex <==
\begin{proof}[Proof of \cref{lem:equalS}]
Define 
\begin{align}
T^+&\coloneqq\{t:
(1+\epsilon)|X_{1,t}|\le |X_{0,t}|
\},\\
T^-&\coloneqq\{t:
|X_{0,t}|\le(1-\epsilon)|X_{1,t}|
\}.
\end{align}
In order to show the lemma, we want to show that
\begin{equation}
\sum_{t\in T^+\cup T^-}
\Pr[t]\le\negl(\secp).
\end{equation}
To show this, assume that    
\begin{equation}
\sum_{t\in T^+\cup T^-}
\Pr[t]\ge\frac{1}{\poly(\secp)}.
\end{equation}
Then the following computationally-unbounded malicious receiver $\cR^*$ can break the statistical hiding
of the classical bit commitment scheme in \cref{protocol:classical}.
\begin{enumerate}
\item
$\cR^*$ honestly executes the commit phase with $\cS$.
Let $t$ be the transcript obtained in the execution.
    \item 
    If $t\in T^+$, $\cR^*$ outputs 0.
    If $t\in T^-$, $\cR^*$ outputs 1.
    If $t\in T$, $\cR^*$ outputs $0$ with probability $1/2$ and outputs 1 with probability $1/2$.
\end{enumerate}
The probability that $\cR^*$ outputs 0 when $\cS$ commits $b=0$ is
\begin{align}
\Pr[0\gets \cR^*|b=0]
&=\sum_{t\in T^+} \Pr[t|b=0]
+\frac{1}{2}\sum_{t\in T} \Pr[t|b=0]\\
&=\sum_{t\in T^+} \frac{|R_t|}{2^\ell}\frac{|X_{0,t}|}{2^\ell}
+\frac{1}{2}\sum_{t\in T} \frac{|R_t|}{2^\ell}\frac{|X_{0,t}|}{2^\ell}.
\end{align}
The probability that $\cR^*$ outputs 1 when $\cS$ commits $b=1$ is
\begin{align}
\Pr[1\gets \cR^*|b=1]
&=\sum_{t\in T^-} \Pr[t|b=1] 
+\frac{1}{2}\sum_{t\in T} \Pr[t|b=1]\\
&=\sum_{t\in T^-} \frac{|R_t|}{2^\ell}\frac{|X_{1,t}|}{2^{\ell}}
+\frac{1}{2}\sum_{t\in T} \frac{|R_t|}{2^\ell}\frac{|X_{1,t}|}{2^{\ell}}.
\end{align}
Then
\begin{align}
&\frac{1}{2}\Pr[0\gets \cR^*|b=0]
+\frac{1}{2}\Pr[1\gets \cR^*|b=1]\\
&=
\frac{1}{2}\sum_{t\in T^+}\Pr[t|b=0]
+\frac{1}{4}\sum_{t\in T}\Pr[t|b=0]
+\frac{1}{2}\sum_{t\in T^-}\Pr[t|b=1]
+\frac{1}{4}\sum_{t\in T}\Pr[t|b=1]\\
&=
\frac{1}{2}\sum_{t\in T^+}\Pr[t|b=0]
+\frac{1}{2}\sum_{t\in T^-}\Pr[t|b=1]\\
&+\frac{1}{4}\Big(1-\sum_{t\in T^+}\Pr[t|b=0]-\sum_{t\in T^-}\Pr[t|b=0]\Big)
+\frac{1}{4}\Big(1-\sum_{t\in T^+}\Pr[t|b=1]-\sum_{t\in T^-}\Pr[t|b=1]\Big)\\
&=
\frac{1}{2}+
\frac{1}{4}\sum_{t\in T^+}(\Pr[t|b=0]-\Pr[t|b=1])
+\frac{1}{4}\sum_{t\in T^-}(\Pr[t|b=1]-\Pr[t|b=0])\\
&=\frac{1}{2}
+\frac{1}{4}\sum_{t\in T^+}\frac{|R_t|}{2^\ell}\frac{|X_{0,t}|-|X_{1,t}|}{2^\ell}
+\frac{1}{4}\sum_{t\in T^-}\frac{|R_t|}{2^\ell}\frac{|X_{1,t}|-|X_{0,t}|}{2^\ell}\\
&\ge\frac{1}{2}
+\frac{1}{4}\sum_{t\in T^+}\frac{|R_t|}{2^\ell}\frac{|X_{0,t}|-\frac{|X_{0,t}|}{1+\epsilon}}{2^\ell}
+\frac{1}{4}\sum_{t\in T^-}\frac{|R_t|}{2^\ell}\frac{|X_{1,t}|-(1-\epsilon)|X_{1,t}|}{2^\ell}\\
&=\frac{1}{2}
+\frac{1}{4}\Big(1-\frac{1}{1+\epsilon}\Big)\sum_{t\in T^+}\frac{|R_t|}{2^\ell}\frac{|X_{0,t}|}{2^\ell}
+\frac{\epsilon}{4}\sum_{t\in T^-}\frac{|R_t|}{2^\ell}\frac{|X_{1,t}|}{2^\ell}\\
&=\frac{1}{2}
+\frac{1}{4}\frac{\epsilon}{1+\epsilon}\sum_{t\in T^+}\frac{|R_t|}{2^\ell}\frac{2|X_{0,t}|}{2^{\ell+1}}
+\frac{\epsilon}{4}\sum_{t\in T^-}\frac{|R_t|}{2^\ell}\frac{2|X_{1,t}|}{2^{\ell+1}}\\
&\ge\frac{1}{2}
+\frac{1}{4}\frac{\epsilon}{1+\epsilon}\sum_{t\in T^+}\frac{|R_t|}{2^\ell}\frac{|X_{0,t}|+|X_{1,t}|}{2^{\ell+1}}
+\frac{\epsilon}{4}\sum_{t\in T^-}\frac{|R_t|}{2^\ell}\frac{|X_{0,t}|+|X_{1,t}|}{2^{\ell+1}}\\
&\ge\frac{1}{2}
+\frac{1}{4}\frac{\epsilon}{1+\epsilon}\sum_{t\in T^+}\frac{|R_t|}{2^\ell}\frac{|X_{0,t}|+|X_{1,t}|}{2^{\ell+1}}
+\frac{\epsilon}{4(1+\epsilon)}\sum_{t\in T^-}\frac{|R_t|}{2^\ell}\frac{|X_{0,t}|+|X_{1,t}|}{2^{\ell+1}}\\
&=\frac{1}{2}
+\frac{1}{4}\frac{\epsilon}{1+\epsilon}\sum_{t\in T^+\cup T^-}\frac{|R_t|}{2^\ell}\frac{|X_{0,t}|+|X_{1,t}|}{2^{\ell+1}}\\
&=\frac{1}{2}
+\frac{1}{4}\frac{\epsilon}{1+\epsilon}
\sum_{t\in T^+\cup T^-}\Pr[t]\\
&\ge\frac{1}{2}+
\frac{1}{4}\frac{\epsilon}{1+\epsilon}
\frac{1}{\poly(\secp)}\\
&=\frac{1}{2}+
\frac{1}{\poly(\secp)},
\end{align}
which breaks the statistical hiding.
\end{proof}



==> backup_coherent_algorithm.tex <==
\begin{figure}[!t]
\begin{algorithm}[H]
\caption{Coherent execution of the commit phase of a classical bit commitment scheme}
\label{protocol:coherent}
\begin{enumerate}
\item
The sender $\cS$ takes $1^\secp$ as input.
The receiver $\cR$ takes $1^\secp$ as input.
    \item 
    $\cR$ samples a random seed $r\gets\bit^\ell$. 
    \item
    $\cS$ generates the state $\sum_{b\in\bit}\sum_{x\in\bit^\ell}\ket{b}\ket{x}\ket{f_1(b,x)}$,
    and measures the third register in the computational basis to obtain the measurement result $\alpha_1$.
    The post-measurement state is
    $\sum_{b\in\bit}\sum_{x\in\bit^\ell,f_1(b,x)=\alpha_1}\ket{b}\ket{x}$.
    $\cS$ sends $\alpha_1$ to $\cR$.
    \item
    $\cR$ computes $\beta_1\coloneqq g_1(r,\alpha_1)$, and sends $\beta_1$ to $\cS$.
    \item
    Let $L$ be the number of rounds. For $j=2$ to $L$, $\cS$ and $\cR$ repeat the following.
    \begin{enumerate}
        \item 
         $\cS$ possesses the state
    \begin{equation}
    \sum_{b\in\bit}\sum_{x\in \cap_{i=0}^{j-1}X_{b}^i}\ket{b}\ket{x}, 
    \end{equation}
    where 
    \begin{align}
     X_{b}^0&\coloneqq\bit^\ell,\\ 
     X_{b}^1&\coloneqq\{x\in \bit^\ell:f_1(b,x)=\alpha_1\}, 
    \end{align}
    and
    \begin{equation}
     X_{b}^i\coloneqq\{x\in\bit^\ell:f_i(b,x,\alpha_1,\alpha_2,...,\alpha_{i-1},\beta_{i-1})=\alpha_i\}   
    \end{equation}
    for $i\ge2$.
\item
      $\cS$ generates the state
    \begin{equation}
    \sum_{b\in\bit}\sum_{x\in \cap_{i=0}^{j-1}X_{b}^i}\ket{b}\ket{x}\ket{f_j(b,x,\alpha_1,\beta_1,...,\alpha_{j-1},\beta_{j-1})}, 
    \end{equation}
    and measures the third
    register in the computational basis to obtain the measurement result $\alpha_j$.
    The post-measurement state is 
     \begin{equation}
    \sum_{b\in\bit}\sum_{x\in \cap_{i=0}^j X_{b}^i}\ket{b}\ket{x}. 
    \end{equation}
    $\cS$ sends $\alpha_j$ to $\cR$.
    \item
    $\cR$ computes $\beta_j\coloneqq g_j(r,\alpha_1,\beta_1,...,\alpha_j)$, and sends $\beta_j$ to $\cS$.
    \end{enumerate}
\end{enumerate}
\end{algorithm}
\end{figure}

==> hashlemma.tex <==
\section{Hashing Lemmas}
\label{sec:hashing}
In this section, we show two useful lemmas, \cref{lem:hash} and \cref{lem:hash2}.
\cref{lem:hash} is used to show \cref{lem:hash2}, and
\cref{lem:hash2} is used in the proof of our main result.

\begin{lemma}
\label{lem:hash}
Let $\mathcal{H}\coloneqq\{h:\cX\to\cY\}$
be a pairwise-independent hash family such that $|\cX|\ge2$.
Let $S\subseteq \cX$ be a subset of $\cX$. 
For any $y\in\cY$,
\begin{equation}
\Pr_{h\gets\mathcal{H}}[|S\cap h^{-1}(y)|\ge1]
\ge
\frac{|S|}{|\cY|}-
\frac{|S|^2}{2 |\cY|^2}.
\label{ge}
\end{equation}
\end{lemma}

\begin{proof}[Proof of \cref{lem:hash}]
First, if $|S|=0$, \cref{ge} trivially holds.
Second, let us consider the case when $|S|=1$.
In that case,
\begin{align}
\Pr_{h\gets\mathcal{H}}[|S\cap h^{-1}(y)|\ge1]
&=
\frac{1}{|\cY|}\\
&\ge\frac{1}{|\cY|}-
\frac{1}{2 |\cY|^2}\\
&=\frac{|S|}{|\cY|}-
\frac{|S|^2}{2 |\cY|^2},
\end{align}
and therefore \cref{ge} is satisfied.
Here, the first equality comes from the fact that
the probability that the unique element of $S$ is mapped to $y$ is $1/|\cY|$.

Finally, let us consider the case when $|S|\ge2$.
The following argument is based on \cite{stackexchange}.
First, for each $y\in\cY$,
\begin{align}
\sum_{j=1}^{|S|}j \Pr_{h\gets\mathcal{H}}[|S\cap h^{-1}(y)|=j]
&=\underset{h\gets\mathcal{H}}{\mathbb{E}}[|S\cap h^{-1}(y)|]\\
&=\underset{h\gets\mathcal{H}}{\mathbb{E}}[|\{x\in S: h(x)=y\}|]\\
&=\sum_{x\in S}\Pr_{h\gets\mathcal{H}}[h(x)=y]\\
&=\frac{|S|}{|\cY|}.\label{ext1}
\end{align}
Second,
for each $y\in\cY$,
\begin{align}
\sum_{j=1}^{|S|}(j-1) \Pr_{h\gets\mathcal{H}}[|S\cap h^{-1}(y)|=j]
&\le
\sum_{j=1}^{|S|}{j\choose 2} \Pr_{h\gets\mathcal{H}}[|S\cap h^{-1}(y)|=j]\\
&=\underset{h\gets\mathcal{H}}{\mathbb{E}}\left[{|S\cap h^{-1}(y)|\choose 2}\right]\\
&=\underset{h\gets\mathcal{H}}{\mathbb{E}}[|\{\{x,x'\}\subseteq S:x\neq x', h(x)=h(x')=y\}|]\\
&=\sum_{\{x,x'\}\subseteq S, x\neq x'}\Pr_{h\gets\mathcal{H}}[h(x)=h(x')=y]\\
&=\frac{1}{|\cY|^2}{|S|\choose2}\\
&=\frac{|S|(|S|-1)}{2 |\cY|^2}\\
&\le\frac{|S|^2}{2 |\cY|^2}.\label{ext2}
\end{align}
(Note that ${n\choose m}=0$ for any $n<m$.)
By extracting both sides of \cref{ext1} and \cref{ext2},
we have
\begin{eqnarray}
\sum_{j=1}^{|S|}    
\Pr_{h\gets\mathcal{H}}[|S\cap h^{-1}(y)|=j]    
&\ge&
\frac{|S|}{|\cY|}-
\frac{|S|^2}{2 |\cY|^2},
\end{eqnarray}
which shows \cref{lem:hash}.
\end{proof}

\begin{lemma}
\label{lem:hash2}
Let $\mathcal{H}\coloneqq\{h:\cX\to\cY\}$
be a pairwise-independent hash family such that $|\cX|\ge2$.
Let $S\subseteq\cX$ be a subset of $\cX$.
For any $y\in\cY$,
\begin{equation}
\Pr_{h\gets\mathcal{H}}[|S\cap h^{-1}(y)|=1]\ge
\frac{|S|}{|\cY|}
-\frac{|S|^2}{|\cY|^2}.
\label{ge2}
\end{equation}
\end{lemma}

\begin{proof}[Proof of \cref{lem:hash2}]
For any $y\in \cY$,
\begin{align}
\frac{|S|}{|\cY|}
&=
\sum_{j=1}^{|S|}j \Pr_{h\gets\mathcal{H}}[|S\cap h^{-1}(y)|=j]\\
&\ge
\Pr_{h\gets\mathcal{H}}[|S\cap h^{-1}(y)|= 1]
+2\Pr_{h\gets\mathcal{H}}[|S\cap h^{-1}(y)|\ge2]\\
&=
2\Pr_{h\gets\mathcal{H}}[|S\cap h^{-1}(y)|\ge1]
-\Pr_{h\gets\mathcal{H}}[|S\cap h^{-1}(y)|=1]\\
&\ge
\frac{2|S|}{|\cY|}-
\frac{|S|^2}{|\cY|^2}
-\Pr_{h\gets\mathcal{H}}[|S\cap h^{-1}(y)|=1].
\end{align}
Here, 
the first equality is from \cref{ext1},
and in the last inequality we have used \cref{lem:hash}.
Therefore,
\begin{align}
\Pr_{h\gets\mathcal{H}}[|S\cap h^{-1}(y)|=1]
&\ge
\frac{2|S|}{|\cY|}-
\frac{|S|^2}{|\cY|^2}
-\frac{|S|}{|\cY|}\\
&=
\frac{|S|}{|\cY|}
-\frac{|S|^2}{|\cY|^2},
\end{align}
which shows \cref{lem:hash2}.
\end{proof}


==> parallel_repetition.tex <==
\section{Parallel Repetition}
\takashi{I found that my idea doesn't work. I'll remove this section if I cannot fix the issue.}
In this section, we show that we can amplify the completeness-soundness gap to be almost optimal by parallel repetition. We focus on the plain (i.e., non-auxiliary-input) version, but the proof can be extended to the auxiliary-input version in a straightforward manner. 
We remark that we cannot rely on existing parallel repetition theorems for interactive arguments because our verifier is inefficient in the second phase. Indeed, it is observed in ?? that parallel repetition may fail even for two-round arguments if the verification is inefficient. 
Even worse, it is even unclear if sequential repetition works for general PoQIV because of the inefficiency of verification while it always works for any interactive arguments with efficient verification. (But we have a relatively simple sufficient condition for PoQIV so that sequential repetition works; see Appendix ??.)
For this reason, we show parallel repetition theorem that is specific to our construction. 


For ease of presentation, we first present an abstracted description of our protocol in ?? and call it $\Pi$.
The first phase is divided into the preamble phase (that corresponds to ?? of ??) and challenge-response phase (that corresponds to ?? and ??) and the second phase is also called the decision phase. In Section ??, we proved that $\Pi$ satisfies $c$-completeness and $s$-soundness where $c-s=1/p(\secp)$ for some polynomial $p$.  
Then the $N$-parallel version $\Pi^N$ of $\Pi$ is described in Figure ??.
We prove the following:
\begin{theorem}\label{thm:para}
If $N\ge \secp\cdot p(\secp)$ \takashi{to be confirmed}, $\Pi^N$ satisfies $(1-\negl(\secp))$-completeness and $\negl(\secp)$-soundness. 
\end{theorem}



\begin{figure}[!t]
\begin{algorithm}[H]
\caption{The abstracted description of our PoQIV $\Pi$}
\label{protocol:abstract_PoQ}
\centering{\bf The first phase}
\begin{enumerate}
\item[\bf Preamble phase:] 
The QPT prover $\cP$ and PPT verifier $\cV_1$ interact with each other to generate a transcript $\tau$. 
\item[\bf Challenge-response phase:]
For $j=1,2$, do the following:
\begin{enumerate}
\item $\cV_1$  chooses $c^j\gets \bit^\ell$ and sends $c^j$ to $\cP$
\item $\cP$ returns a response $a^j$ to $\cV_1$. 
\end{enumerate}
\end{enumerate}
\centering{\bf The second phase}
\begin{itemize}
\item[\bf Decision phase] The unbounded-time $\cV_2$ takes a transcript $I=(\tau,c^1,a^1,c^2,a^2)$ of the first phase as input and outputs $\top$ or $\bot$. 
\end{itemize}
\end{algorithm}
\end{figure}

\begin{figure}[!t]
\begin{algorithm}[H]
\caption{$N$-parallel version $\Pi^N$ of $\Pi$}
\label{protocol:para_abstract_PoQ}
\centering{\bf The first phase}
\begin{enumerate}
\item[\bf Preamble phase:] 
The QPT prover $\cP$ and PPT verifier $\cV_1$ 
run $N$ parallel copies of the preamble phase of $\Pi$ to generate a transcript $\vtau=(\tau_1,\ldots,\tau_N)$. 
\item[\bf Challenge-response phase:]
For $j=1,2$, do the following:
\begin{enumerate}
\item For $i\in [N]$, $\cV_1$  chooses $c_{i,j}\gets \bit^\ell$ and sends $c_{i,j}$ to $\cP$
\item 
For $i\in [N]$,  $\cP$ returns a response $a_{i,j}$ to $\cV_1$ where $a_{i,j}$ is generated as in $\Pi$. 
\end{enumerate}
\end{enumerate}
\centering{\bf The second phase}
\begin{itemize}
\item[\bf Decision phase:] The unbounded-time $\cV_2$ takes a transcript $\vI=\{I_i=(\tau_i,c_{i}^{1},a_{i,1},c_{i}^{2},a_{i,2})\}_{i\in [N]}$ of the first phase as input. 
For $i\in [N]$, 
it runs $\cV_2$ of $\Pi$ on $I_i$ and sets $X_i\seteq 1$ if it accepts and otherwise sets $X_i\seteq 0$. 
If $\frac{\sum_{i\in [N]}X_i}{N}>\frac{c+s}{2}$, 
it outputs $\top$ and otherwise outputs $\bot$. 
\end{itemize}
\end{algorithm}
\end{figure}

\subsection{Proof of \cref{thm:para}}
\takashi{not completed yet}
First, $(1-\negl(\secp))$-completeness immediately follows from $N\ge \secp \cdot p(\secp)$ and Chernoff bound. 
In the following, we prove $\negl(\secp)$-soundness. 

Suppose that $\Pi^N$ does not satisfy $\negl(\secp)$-soundness. Then there is a PPT algorithm $\cP^*$ and
polynomial $\poly$ such that  
\begin{align}
\Pr[\cV_2(\vI)\rightarrow \top:\vI \gets \langle \cP^*,\cV_1 \rangle(1^\secp)]\ge \frac{1}{\poly(\secp)}.
\end{align}
By a similar averaging argument to that for the stand-alone case (proof of Theorem ??), we only have to consider the case where $\cP^*$ is deterministic. \takashi{I'll write that later.}

We define several notations.
We call $\vc^1$ and $\vc^2$ the first and second challenges, respectively.
For $j\in \{1,2\}$, we define
\begin{align}
\vc^{j}\seteq (c_{1}^{j},\ldots,c_{N}^{j}).
\end{align} 
For $i\in [N]$ and $j\in \{1,2\}$, we define 
\begin{align}
\vc_{-i}^{j}\seteq (c_{1}^{j},\ldots,c_{i-1}^{j},c_{i+1}^{j},\ldots,c_{N}^{j}).
\end{align}
For $\vtau$  and $\vc^1\in \bit^{\ell\times N}$, we write $\vI \gets \langle \cP^*,\cV_1 \rangle(\vtau,\vc^1)$
to mean to run the interaction between $\cP^*$ and $\cV_1$ where the transcript of the preamble phase is fixed to $\vtau$ and the first challenge is fixed to $\vc^1$ 
and generate the transcript $\vI$.
Similarly, for $\vtau$  and $\vc^1,\vc^2\in \bit^{\ell\times N}$, we write $\vI \gets \langle \cP^*,\cV_1 \rangle(\vtau,\vc^1,\vc^2)$
to mean to run the interaction between $\cP^*$ and $\cV_1$ where the transcript of the preamble phase is fixed to $\vtau$ and the first and second challenges are fixed to $\vc^1$ and $\vc^2$, respectively,  
and generate the transcript $\vI$.

For each $\vtau$, 
$i\in [N]$, and $c_{i}^{1}\in \bit^\ell$, we define a probability $P[\vtau,i,c_{i}^{1}]$ as follows:
\begin{align}
P[\vtau,i,c_{i}^{1}]\seteq \Pr[
\cV_2(\vI)\rightarrow \top
:
\vc_{-i}^{1}\gets \bit^{\ell\times (N-1)}, 
\vI \gets \langle \cP^*,\cV_1 \rangle(\vtau,\vc^1)].
\end{align}
Similarly, for each $\vtau$, 
$\vc^1\in \bit^{\ell\times N}$, 
$i\in [N]$,  
and $c_{i}^{2}\in \bit^\ell$, we define a probability $P[\vtau,\vc^1,i,c_{i}^{2}]$ as follows:
\begin{align}
P[\vtau,\vc^1,i,c_{i}^{2}]\seteq \Pr[
\cV_2(\vI)\rightarrow \top
:
\vc_{-i}^{2}\gets \bit^{\ell\times (N-1)}, 
\vI \gets \langle \cP^*,\cV_1 \rangle(\vtau,\vc^1,\vc^2)].
\end{align}

For each $\vtau$, 
$i\in [N]$, and $c_{i}^{1}\in \bit^\ell$, we 
define a subset $\GC[\vtau,i,c_{i}^{1}]\subseteq \bit^{\ell}$ 
to be the set consisting of $\epsilon$-fraction of $c_{i}^{1}\in \bit^{\ell}$ with the highest probability $P[\vtau,i,c_{i}^{1}]$ where $\epsilon \seteq \frac{1}{4N\poly(\secp)}$. \takashi{$P[\vtau,i,c_{i}^{1}]$ ga ookii hou kara jun ni $\epsilon$-fraction wo erabu to iu imi. I don't know how to properly write this in English right now, I'll think about this later.}
Similarly,  for each $\vtau$, $\vc^1\in \bit^{\ell\times N}$,   
$i\in [N]$, and $c_{i}^{1}\in \bit^\ell$, we 
define a subset $\GC[\vtau,\vc^1,i,c_{i}^{2}]\subseteq \bit^{\ell}$ 
to be the set consisting of $\epsilon$-fraction of $c_{i}^{2}\in \bit^{\ell}$ with the highest probability $P[\vtau,\vc^1,i,c_{i}^{2}]$. 

For each $i\in [N]$, we define a cheating prover $\widetilde{\cP}_i^*$ against $\Pi$ that works as follows:
\begin{enumerate}
\item In the preamble phase, 
$\overline{\cP}^*_i$ works similarly to $\cP^*$  where it embeds the messages from the external verifier of $\Pi$ into the $i$-th copy of $\Pi$ and simulates messages of all the other copies by itself. Let $\vtau$ be the transcript in this phase.
\item Upon receiving the first challenge $c^1$,
$\widetilde{\cP}^*_i$ 
sets $c_i^1\seteq c^1$, 
samples $\vc_{-i}^1\gets \bit^{\ell\times (N-1)}$,
passes $\vc^1= (c_1^1,\ldots,c_N^1)$ to $\cP^*$ as the first challenge of $\Pi^N$, receives $\va^1=(a_1^1,\ldots,a_N^1)$ from $\cP^*$ and sends 
it works similarly to $\cP^*$.
\item Upon receiving the second challenge $\vc^2$, $\overline{\cP}^*_i$ immediately aborts if there is $i\in [N]$ such that  $c_i^2\in \GC[\vtau,\vc^1,i,c_{i}^{2}]$. Otherwise, it works similarly to $\cP^*$.
\end{enumerate}


We define a modified {\it inefficient} cheating prover $\overline{\cP}^*$ against $\Pi^N$ that receives "good challenges". 
Formally, it works as follows:
\begin{enumerate}
\item In the preamble phase, 
$\overline{\cP}^*_i$ works similarly to $\cP^*$. Let $\vtau$ be the transcript in this phase.
\item Upon receiving the first challenge $\vc^1$, $\overline{\cP}^*_i$ immediately aborts if there is $i\in [N]$ such that  $c_i^1\in \GC[\vtau,i,c_{i}^{1}]$. Otherwise, it works similarly to $\cP^*$.
\item Upon receiving the second challenge $\vc^2$, $\overline{\cP}^*_i$ immediately aborts if there is $i\in [N]$ such that  $c_i^2\in \GC[\vtau,\vc^1,i,c_{i}^{2}]$. Otherwise, it works similarly to $\cP^*$.
\end{enumerate}

\begin{proposition}
\begin{align}
\Pr[\cV_2(\vI)\rightarrow \top:\vI \gets \langle \overline{\cP}^*,\cV_1 \rangle(1^\secp)]\ge \frac{1}{2\poly(\secp)}.
\end{align}
\end{proposition}
\begin{proof}
For each $i\in [N]$, 
\begin{align}
\Pr[c_i^1\in \GC[\vtau,i,c_{i}^{1}]]\le \epsilon
\end{align}
and 
\begin{align}
\Pr[c_i^2\in \GC[\vtau,\vc_1,i,c_{i}^{2}]]\le \epsilon.
\end{align}
Thus by the union bound, the probability that $\overline{\cP}^*$ aborts is at most $2N\epsilon = \frac{1}{\poly(\secp)}$. 
Since $\overline{\cP}^*$  works similarly to $\cP^*$ if it does not abort, the proposition follows from Eq??. 
\end{proof}

For each $i\in [N]$, we define the following {\it inefficient} cheating prover $\cP^*_i$ against the stand-alone protocol $\Pi$:
\begin{enumerate}
\item 
In the preamble phase, 
$\cP^*_i$ runs similarly to $\cP$ where it embeds the messages from the external verifier of $\Pi$ into the $i$-th copy of $\Pi$ and simulates messages of all the other copies by itself.
\item Upon receiving the first $c^1$ from the external verifier, 
\end{enumerate}

==> worst_case.tex <==
\section{Complexity Theoretic Implication}
In this section, we discuss complexity theoretic implication.

\subsection{Definitions}
Intuitively, the existence of proofs of quantumness with inefficient verification can be viewed as ``interactive quantum advantage''. For formally studying it,   
we define ``interactive'' versions of $\mathbf{SampBQP}$ and $\mathbf{SampBPP}$. 
\begin{definition}
An interactive sampling problem is a collection $((D_x)_{x\in \bit^*},V)$ where $D_x$ is a distribution over $\bit^{p(|x|)}$ for a fixed polynomial $p$ for all $x\in \bit^*$ and $V$ is an interactive classical Turing machine. 
$\mathbf{IntSampBPP}$ is the class of interactive sampling problems $((D_x)_{x\in \bit^*},V)$ for which there is a PPT algorithm $\A$ such that 
\begin{align}
\Delta(\langle\A(1^{\epsilon^{-1}}),V\rangle(x),D_x) \le \epsilon 
\end{align}
for all $\epsilon$ and $x$
where $\langle\A(1^{\epsilon^{-1}}),V\rangle(x)$ is the distribution of a transcript of interaction between $\A$  and $V$ with common input $x$ and $\A$'s private input $1^{\epsilon^{-1}}$. 
For a function $N:\mathbb{N}\rightarrow \mathbb{N}$, we define the subclass $\mathbf{IntSampBPP}_N\subseteq \mathbf{IntSampBPP}$ to be the class of interactive sampling problems that satisfies the above and the number of messages exchanged between $\A$ and $V$ is at most $N(|x|)$.  
$\mathbf{IntSampBQP}$ and $\mathbf{IntSampBQP}_{N}$ are defined similarly except that $\A$ is a QPT algorithm but the communication is still classical.  
\end{definition}
By using the above definition, we can interpret $\mathbf{IntSampBPP}_N\neq \mathbf{IntSampBQP}_N$ as ``quantum advantage'' in the $N$-round interactive setting. 
Here are several remarks.
\begin{remark}
We have $\bigcup_{c\in \mathbb{N}}\mathbf{IntSampBPP}_{|x|^c}=\mathbf{IntSampBPP}$ and $\bigcup_{c\in \mathbb{N}}\mathbf{IntSampBQP}_{|x|^c}=\mathbf{IntSampBQP}$ where we abuse the notation to write $|x|^c$ to mean a function that maps $|x|$ to $|x|^c$. This is because we require $\A$ to be PPT or QPT and in particular the number of interaction must be polynomial. 
\end{remark}
\begin{remark}
For any $N,N'$ such that $N(|x|)\le N'(|x|)$ for all $x$,  $\mathbf{IntSampBPP}_N\neq \mathbf{IntSampBQP}_N$ implies $\mathbf{IntSampBPP}_{N'}\neq \mathbf{IntSampBQP}_{N'}$
\end{remark}
\begin{remark}
The classes $\mathbf{SampBPP}$ and  $\mathbf{IntSampBPP}_1$ are ``equivalent'' in the following sense: 
 For any  sampling problem $(D_x)_{x\in \bit^*}$, we have $(D_x)_{x\in \bit^*}\in \mathbf{SampBPP}$ if and only if $((D_x)_{x\in \bit^*},V_{\mathsf{null}})\in \mathbf{IntSampBPP}_1$ where $V_{\mathsf{null}}$ is a trivial interactive Turing machine that does not send anything and only receive a single message. Moreover, any interactive sampling problem in $\mathbf{IntSampBPP}_1$ must be of the above form and thus it naturally gives a sampling problem in $\mathbf{SampBPP}$. 
 A similar ``equivalence'' holds for $\mathbf{SampBQP}$ and  $\mathbf{IntSampBQP}_1$. Therefore, 
 we have $\mathbf{SampBPP}\neq  \mathbf{SampBQP}$ if and only if $\mathbf{IntSampBPP}_1\neq \mathbf{IntSampBQP}_1$. 
 In particular, $\mathbf{SampBPP}\neq  \mathbf{SampBQP}$ implies $\mathbf{IntSampBPP}\neq \mathbf{IntSampBQP}$.
 On the other hand, the other direction is unlikely to hold by the oracle separation shown in \cref{cor:separation_intsamp}.
\end{remark}


\subsection{Sufficient Conditions for Interactive Quantum Advantage}
It is easy to see that the existence of auxiliary-input proofs of quantumness with inefficient verification implies $\mathbf{IntSampBPP} \neq  \mathbf{IntSampBQP}$. 
\begin{theorem}
If there exist $N$-round auxiliary-input proofs of quantumness with inefficient verification, then $\mathbf{IntSampBPP}_{N} \neq  \mathbf{IntSampBQP}_{N}$. 
%Moreover, if the auxiliary-input proofs of quantumness with inefficient verification is constant-round, then $\mathbf{IntSampBPP}_{O(1)} \neq  \mathbf{IntSampBQP}_{O(1)}$. 
\end{theorem}
\begin{proof}
\takashi{I believe it is easy.}
\end{proof}

As shown in ??, 
$N$-round auxiliary-input statistically hiding and computationally binding commitments imply
$N+6$-round auxiliary-input proofs of quantumness with inefficient verification. We have the following instantiations for such commitments:
\begin{itemize}
\item Instantiation of the poly-round commitment scheme of \cite{SIAM:HNORV09} with auxiliary-input one-way functions instead of one-way functions. Note that auxiliary-input one-way functions exist if $\mathbf{BPP}\neq \mathbf{CZK}$~\cite{OW93}. 
\item Instantiation of the $2$-round commitment scheme of \cite{C:HalMic96} with auxiliary-input collision-resistant hash functions instead of collision-resistant hash functions. Note that auxiliary-input collision-resistant hash functions if and only if   $\mathbf{PWPP}\nsubseteq \mathbf{FBPP}$ as shown in Appendix ??. 
\item A non-interactive scheme based on the assumption  $\mathbf{BPP}\neq \mathbf{SZK}$ as shown in Appendix ??.
\end{itemize}
We omit the details for the first two constructions because their constructions and security proofs are identical to those of  \cite{SIAM:HNORV09} and \cite{C:HalMic96}, respectively except that we additionally consider auxiliary inputs.  
Then we obtain the following corollaries which give complexity theoretic charactirization for $\mathbf{IntSampBPP} \neq  \mathbf{IntSampBQP}$ and $\mathbf{IntSampBPP}_{O(1)} \neq  \mathbf{IntSampBQP}_{O(1)}$.
\begin{corollary}
If $\mathbf{BPP}\neq \mathbf{CZK}$, then $\mathbf{IntSampBPP} \neq  \mathbf{IntSampBQP}$.
\end{corollary}
\begin{corollary}
If $\mathbf{PWPP}\nsubseteq \mathbf{FBPP}$, then $\mathbf{IntSampBPP}_{8} \neq  \mathbf{IntSampBQP}_{8}$.
\end{corollary}
\begin{corollary}
If $\mathbf{BPP}\neq \mathbf{SZK}$, then $\mathbf{IntSampBPP}_{7} \neq  \mathbf{IntSampBQP}_{7}$.
\end{corollary}

\subsection{Necessary Conditions for Interactive Quantum Advantage}
We show that an unconditional proof of $\mathbf{IntSampBPP} \neq  \mathbf{IntSampBQP}$ is hopeless. 

\takashi{
I hope we can prove the following theorem.
\begin{theorem}
If $\mathbf{BPP}= \mathbf{PP}$, then
$\mathbf{IntSampBPP} =  \mathbf{IntSampBQP}$.
\end{theorem}
I'm not sure if we can prove the above theorem.
But if we strengthen the assumption to $\mathbf{BPP}= \mathbf{PSPACE}$, then that seems easy to prove.
}


\subsection{Oracle Separations}
We showed interactive quantum advantage exists assuming the existence of one-way functions. Can we show non-interactive quantum advantage from the same assumption? We show that this is not possible at least in the relativized setting. 
\begin{theorem}\label{thm:separation_samp_OWF}
There is an oracle relative to which  $\mathbf{SampBPP}= \mathbf{SampBQP}$
but one-way functions exist. 
\end{theorem}
\begin{corollary}\label{cor:separation_intsamp}
There is an oracle relative to which   $\mathbf{SampBPP}= \mathbf{SampBQP}$
but $\mathbf{IntSampBPP} \neq  \mathbf{IntSampBQP}$. 
\end{corollary}
\takashi{define $\mathcal{O}$ to be a pair of $\mathbf{SampBQP}$ oracle and random oracle.}

\takashi{I'm wondering if we can prove the following theorem.
\begin{theorem}
There is an oracle relative to which $\mathbf{IntSampBPP} =  \mathbf{IntSampBQP}$ but $\mathbf{BPP}\neq \mathbf{NP}$
\end{theorem} 
If this is true, this can be seen as an evidence of the difficulty of weakening the assumption to  $\mathbf{BPP}\neq \mathbf{NP}$.
(Note that this does not contradict my original claim since $\mathbf{IntSampBPP}$ and $\mathbf{IntSampBQP}$ are defined w.r.t. additive errors.)
}
